AltCanvas: A Tile-Based Image Editor with Generative AI for Blind or Visually Impaired People

People with visual impairments often struggle to create content that relies heavily on visual elements, particularly when conveying spatial and structural information. Existing accessible drawing tools, which construct images line by line, are suitable for simple tasks like math but not for more expressive artwork. On the other hand, emerging generative AI-based text-to-image tools can produce expressive illustrations from descriptions in natural language, but they lack precise control over image composition and properties. To address this gap, our work integrates generative AI with a constructive approach that provides users with enhanced control and editing capabilities. Our system, AltCanvas, features a tile-based interface enabling users to construct visual scenes incrementally, with each tile representing an object within the scene. Users can add, edit, move, and arrange objects while receiving speech and audio feedback. Once completed, the scene can be rendered as a color illustration or as a vector for tactile graphic generation. Involving 14 blind or low-vision users in design and evaluation, we found that participants effectively used the AltCanvas workflow to create illustrations.

==> 11_alttext.tex <==
teaser figure
A diagram of AltCanvas' three steps image authoring steps. A on the left: The tile-based interface can add images by talking to them. B in the middle: Images can be edited through sonification, verbal feedback, and arrow keys. C on the right: The rendering process of black-and-white and color graphics. Step A: It shows a tile-based interface with a highlighted square, suggesting the selection of a tile, and an instruction bubble that reads, "Add an image of a running dog," prompting the start of the image generation. Step B: The interface now includes a line drawing of a running dog next to a ball, with a directional arrow indicating the ability to move the ball. Below, there's a legend explaining the editing controls, such as using arrow keys to adjust the location of objects. Step C: This step is divided into two parts. The upper part shows the final black-and-white tactile graphic, a simple and clear line drawing of a dog chasing a flying disc with a tree in the background. The lower part displays the color graphic with final rendering, where the same scene is depicted in full color with a blue sky, a lush green tree, and the dog joyfully leaping towards the blue flying disc.


  \label{fig:formative}
  \Description{The participants' previous works including a pen and crayon drawing, the original grid layout for placing images, and an artwork of a bridge written in SVG code. From the left, P2 showed us drawings using ballpoint pens and crayola crayons on paper. P3 showed us the process of using a grid layout to create shape cutouts. On the right, P5 showed us an example artwork of the Golden Gate Bridge using SVG Code. From the right there is an image created by P2 | A sketched artwork of three figures, possibly a family, with two larger figures and a smaller one in the middle. They appear to be dancing or interacting playfully. The image is created with ballpoint pen and colored with Crayola crayons on paper. P3 | A photo of a hands-on crafting process showing a black greeting card with a cut-out pattern placed on a white grid layout. The card features a star-like pattern made from the cut-outs. P5 | A digital illustration of a red suspension bridge, possibly resembling the Golden Gate Bridge, against a white background. This artwork is noted as being created by writing SVG code.}

  \label{table_user}
  \Description{  This table summarizes the characteristics of participants across three different studies focused on formative need finding, design feedback, and user evaluation. It consists of six columns: Participant ID (P1 through P14), Eyesight status (Blind or Low Vision), Past Experience (Expert or Novice), and three columns indicating participation in Interviews, Design Study, and Evaluation with 'yes' or 'no' responses. Participants P1 to P5 are blind experts and have participated in interviews, but their participation varies in design studies and evaluations. Participants P6 to P11 are a mix of blind or low vision novices, with varying participation in the design study and evaluation but no interviews. The last three participants (P12 to P14) are novices with different eyesight statuses and have only participated in the evaluation.}

\label{fig:ux_onLoad}
    \Description{ A series of interface screenshots labeled from A to D illustrate different sections of the AltCanvas. A. Region of the Tile Based Interface. B. Region of the Canvas Interface. C. Region of the Keyboard shortcut commands D. System Settings with Image Style and Speech Speed. The screen D will pop up initially for the user for settings. Users can access the keyboard commands screen C when pressing SHIFT + K. Users can navigate through the screen A and B region while editing the image. In part A, titled "TileRegion" has a matrix of tiles, which are used to select and place images within the canvas. The tile currently selected is highlighted. Part B, called "Canvas Region," displays a canvas area with a 600x600 pixel grid where a line drawing of a running dog and a tree has been placed. Part C features a pop-up window with "Keyboard Instructions," listing shortcuts like 'Shift + K' for keyboard command instructions, and other combinations for various editing actions. Finally, part D shows the "System Settings" window, where users can adjust the canvas size width and height, image style between tactile and color graphics and control speech speed for audio feedback.

    

    \label{fig:ux_describe}
    \Description{ The two screenshots of interface to describe the AltCanvas's image descriptions. On the left, A. Global Description of the canvas is available. The user can press the SHIFT +G command to hear the global description of the canvas. On the right, B. Local Description activates the local information explanation by pressing the SHIFT +I command. This will describe the image on the current tile to the user. C. The Image Chat function. This command can be accessed through SHIFT +C. This feature will answer the question the user asks about the image on the current tile. In detail, the section A displays the 'Global Canvas Description' where a user has given a general description of a scene featuring a dog leaping towards the left to catch a frisbee, with a tree to the right of the dog. In section B, called 'Local Canvas Description,' there's a focused description of a particular element dubbed 'dog.' It describes the dog's action, the art style, and provides specific coordinates and size for the drawing on the canvas. Section C shows 'Image Chat Mode' where a voice command asking for the appearance of the dog’s tail is given, and the software responds that the tail is narrow, pointy, and pointing upwards.}


 \label{fig:ux_interact}
    \Description{Edit image locations with SHIFT + L and arrow keys: A thump sound indicates edge collision (A), speech notifies object collision (B), spatial sounds and coordinates describe movement (C). SHIFT + S adjusts size with variable frequency tones (D). Tile manipulation and radar scan reveal layout and distances (E, F).
    Panel A features a simple line drawing of a dog in different positions, with a speech bubble indicating sound feedback when interacting with the image.
    Panel B depicts the same dog with a speech bubble saying "Overlapping with Frisbee" to signal a conflict in the image layout.
    Panel C shows an arrow pointing to the right with a speech bubble, and text indicating that the current location is 200 by 300, suggesting a feature to move elements on the canvas.
    Panel D provides audio feedback information where the frequency of the sound increases with the size of the image element, which in this case is a drawing of the dog.
    Panel E has a grid similar to panel A, with a highlighted tile indicating that it has been pushed to the left, showing how to move tiles within the interface.
    Finally, panel F uses a radar scan metaphor to describe the spatial relationship between the elements on the canvas, with the tree being 20 pixels to the right, the frisbee 50 pixels up and 30 pixels left from the dog's position.}
\end{figure*}


    \label{fig:render}
    \Description{The figure shows a two-tiered illustration. Once the user has generated the final image through AltCanvas, the figure depicts the rendering options that are available to the user. The first option is, 'Background Rendering,' The images display four examples of a rendered scene featuring a dog, a tree, and a frisbee (the image the user has generated) in different environments: a sunny day with blue skies, a night scene with a moonlit backdrop, an autumn setting with leaves on the ground, and a dusk scene with a sunset. Each background has a the prompt that the user inputs to generate the final image. The lower tier, 'Edge Detection for Tactile Rendering Option,' presents a black and white outline of the same scene for tactile rendering purposes, with a list of technical options for edge detection algorithms including Sobel and Canny.}



      \label{fig:pilot}
    \Description{ The main four types of interactions that were tested in the pilot study. (A)Tile Navigation: here, we tested if users were able to gain a spatial understanding of the canvas by navigating through the tiles. (B) Global Info, Local Info, here we tested the descriptions of the image to gain an understanding of the different types of descriptions wanted. (C) Location Edit: Here, we studied how users navigated through changing the location of images and the types of information they wanted. (D) Size Edit, here, we studied how users changed the size of objects on the canvas. Panel A is titled "Tile Navigation" and illustrates a grid where each tile represents an element of the image. The panel shows a music note and a sun icon, with a label "Dog" on one of the tiles. A speech bubble indicates that sonification is used for tile navigation and that speech feedback is provided on the image content.
    Panel B is labeled "Global Info, Local Info" and depicts two speech bubbles: one for a local description stating "The dog is facing the left. The image depicts a line drawing." and another for a global description mentioning a sun in the top right corner and a small dog in the center.
    Panel C, "Location Edit," shows an interface where the position of image elements can be edited. A selected tile with a dog is highlighted, and a keyboard shortcut is suggested for editing the location.
    Panel D, "Size Edit," demonstrates how the size of an image element can be adjusted. It shows a tile with a sun, and an arrow icon implies the scaling function, with a keyboard shortcut for size editing mentioned.


       \label{fig:architecture}
    \Description{ Pipeline for Image Generation : The audio of the user is captured and parsed to single out the main components of the prompt using a wink-pos-tagger. The parsed prompt is processed into Tactile Graphic Generation and Visual Color Generation Prompts based on the type of image the user wishes to generate. This final prompt is passed into the image generation model and goes through a verification process based on the initial prompt and image type requirements. The final image is passed through a background removal API and the url is used to generate descriptions of the given image. The image is a flowchart detailing the process of generating an image from an audio recording. The flow starts with an audio recording, which goes through 'Prompt Parsing' where nouns and adjectives are extracted. These extracted words feed into two paths: 'Tactile Graphic Generation Prompt' and 'Visual Color Image Generation Prompt,' both leading into an 'Image Generation Model.' The output of the model is an 'Image Description Generation,' which presumably describes the generated image. This description is linked to 'Saved Images,' suggesting that the generated images are stored. Additionally, there is a 'Background Removal API' that processes the saved images to remove their backgrounds, illustrated by a transition from a full image to one where only the subject remains.}


\label{fig:final_likert}
    \Description{ The image is a bar chart displaying user feedback on a tool, with each statement rated on a Likert scale ranging from "Strongly Disagree" to "Strongly Agree." The vertical y-axis lists user statements, and the horizontal x-axis represents the percentage of responses. Darker shades of blue indicate stronger agreement, while red tones indicate disagreement. The statements, from top to bottom, are: I could easily understand how to use the tool. I want to create more images with this tool. I could easily generate the image using this tool. The voice command feature was intuitive to use. The sonification feature was intuitive to use. The tile-based interface was intuitive to use. I could easily edit the image as I was creating it. I could easily understand the state of the canvas through voice explanations. I could easily understand the state of the canvas through sounds. LIKERT Scale responses for the final study on a 7 point scale. Highest satisfaction can be observed for the questions "I could easily understand how to use this tool" (avg = 6.5, std= 0.75), "The voice command feature was intuitve to use" (avg = 6.5, std=1.06). "The tile based interface was intuitve to use" (avg= 5.8, std=2.03) and "I could easily edit the image as I was creating it"(avg= 6.3, std=0.7). Mixed responses were received for "I want to create more images with this tool"(avg=5, std= 2.3) and "I could easily generate the image using this tool" (avg= 4.8, std=1.3). The primary reason behind this is because of the unreliability of image generations from the AI model. The majority strongly agree that they could easily understand how to use the tool and that the voice command feature was intuitive. Most users agree or strongly agree that they want to create more images with the tool. Opinions vary more on the tile-based interface and the ease of editing images, with a spread across neutral to agree.}


     \label{fig:final_interactions}
    \Description{ The image is a grid-based chart representing the actions taken by participants in two separate tasks. Each row corresponds to a participant labeled P3, P5, P6, P7, P10, P12, P13, and P14. The columns represent different actions: Image Generation (blue), Location Edit (pink), Size Edit (yellow), Image Descriptions (green), and Delete Image (gray). Task 1 and Task 2 are shown in two separate sections of the grid. The participants' actions are marked on the grid with colored squares corresponding to the actions' legend, illustrating the sequence and frequency of each action performed by the participants across the tasks.A visualized Sequence of Edit Interactions for three tasks. The blue refers to image generation tasks, the pink refers to location edits, yellow refers to size edits, green refers to image descriptions, and gray refers to delete image. The boxes correspond to the editing durations. A general trend of global and local image descriptions used after multiple edit interactions and towards the end of image editing can be observed. For task one, a total of three images were generated, whereas in task two, a total of five images have been generated. Image generations are followed by an image delete for incorrect generations. The green image descriptions refer to the separate image description commands accessed by SHIFT +G (Global), SHIFT+I (Information), and SHIFT+C (Chat). The general trend shown in the chart is that participants engage in various image editing activities, with some actions being more common than others. In both Task 1 and Task 2, 'Image Generation' (blue) and 'Location Edit' (pink) are quite prevalent across most participants, indicating these are frequent steps in the tasks. 'Size Edit' (yellow) also appears regularly, but less often than image generation or location editing. 'Image Descriptions' (green) are used moderately throughout, and 'Delete Image' (gray) is the least frequent action, suggesting that participants do not often delete images once they have been generated or edited. The pattern of actions seems consistent between Task 1 and Task 2, indicating similar behavior across tasks by the participants.}



\label{keyboard_command}
\Description{This table lists the 10 main keyboard commands used in a system and their respective functions and interactions. It has three columns: 'Keyboard Commands', 'Function', and 'Main Interaction'. For example, pressing 'ENTER' generates a new image with speech, while 'SHIFT + G' provides a global description of the canvas. Local descriptions, radar scans for nearby objects, image chats, and editing image location or size are performed with various 'SHIFT' plus a letter key combinations. The 'SHIFT + Arrow Key' pushes image tiles, 'SHIFT + X' deletes an image, and the arrow keys alone navigate through tiles. 'ESC' is used to quit or stop actions within the system. Each command aligns with a specific interaction for image editing and navigation within the system, aimed at enhancing user experience.}






    






\subsection{TaskOne: Sample User Graphic Generations}

\Description{The image presents three sample user graphic generations for 'Task One'. Each sample depicts three items: a dog, a dog bowl, and a clock. The first graphic shows a simple, cartoon-style representation with a puppy in front of a dog bowl that has a few pieces of dog food scattered around, and a wall clock with roman numerals above. In the second graphic, there is a more detailed drawing of a dachshund with a wagging tail next to an empty dog bowl, and a wall clock with hands pointing at eleven and one.
The third graphic features a corgi sitting proudly between two dog bowls decorated with paw prints, and a wall clock with a second hand above it.}



\subsection{TaskTwo: Sample User Graphic Generations}

\Description{ The image showcases three sets of line-drawn graphics created by users as part of 'Task Two'. Each set includes a window, a clock, a cat, a table, and a potted plant. In the first graphic, the window is styled with curtains pulled aside, the clock has simple numbers and hands, the cat appears seated and alert, the table is square with a flowerpot that has several flowers.
The second graphic features a grid-style window, a clock with Roman numerals, a lounging cat, and a round table with a large potted plant.
The third graphic depicts an arched window with a divided pane, a clock marked with lines instead of numbers, a fluffy cat seated in front of a slender table supporting a potted plant with long leaves.
Each graphic presents these common elements with varying artistic interpretations, showcasing different styles and details in the users' renditions.}


\subsection{TaskThree: Sample User Graphic Generations}

\Description{
The image is a compilation of three sets of graphics generated by users for 'Task Three'. Each graphic represents a different theme described by the users: The first graphic depicts a family of three (mom, dad, and daughter), standing next to a turtle and a unicorn, showcasing a combination of real and mythical creatures.
The second graphic shows a scene with three items: a decorated Christmas tree, a racing car, and a pickup truck, suggesting a contrast between the stationary and the dynamic.
The third graphic features a playful set with a character that resembles a Minion wearing glasses and holding a spatula grilling things for a barbecue, a round character that could be Kirby floating on water, and a simple basket, highlighting characters from popular culture and a common object.
Each set of images captures unique elements as specified by the users, reflecting their individual creative interpretations of the given task.}

